SWAD: Domain Generalization by Seeking Flat Minima

Domain generalization (DG) methods aim to achieve generalizability to an unseen target domain by using only training data from the source domains. Although a variety of DG methods have been proposed, a recent study shows that under a fair evaluation protocol, called DomainBed, the simple empirical risk minimization (ERM) approach works comparable to or even outperforms previous methods. Unfortunately, simply solving ERM on a complex, non-convex loss function can easily lead to sub-optimal generalizability by seeking sharp minima. In this paper, we theoretically show that finding flat minima results in a smaller domain generalization gap. We also propose a simple yet effective method, named Stochastic Weight Averaging Densely (SWAD), to find flat minima. SWAD finds flatter minima and suffers less from overfitting than does the vanilla SWA by a dense and overfit-aware stochastic weight sampling strategy. SWAD shows state-of-the-art performances on five DG benchmarks, namely PACS, VLCS, OfficeHome, TerraIncognita, and DomainNet, with consistent and large margins of +1.6% averagely on out-of-domain accuracy. We also compare SWAD with conventional generalization methods, such as data augmentation and consistency regularization methods, to verify that the remarkable performance improvements are originated from by seeking flat minima, not from better in-domain generalizability. Last but not least, SWAD is readily adaptable to existing DG methods without modification; the combination of SWAD and an existing DG method further improves DG performances. Source code is available at https://github.com/khanrc/swad.

==> checklist.tex <==
% You should answer yes, no, or n/a.
% You should reference the section(s) of the paper that provide support for your answer.
% You can also optionally write a short (1–2 sentence) justification of your answer.

\section*{Checklist}



\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section 5 in the main text.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Appendix.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{See Appendix. While we use public datasets only, we track how the datasets were built to discuss their potential ethical issue.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See Section 2 in the main text and more precise assumptions are stated in Appendix.}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{Proofs can be found in the supplementary material. We omit the entire proofs in the main manuscript due to the limitation of space.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We provide the code publicly to reproduce our main results. The code include the instructions to download data and to reproduce the results.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We provide about the data splits, how they were chosen, and important hyperparameters in the Section 4 of the main text. Further details are provided in Appendix and the code.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We report the standard error from three runs, following~\citet{gulrajani2020domainbed}.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix. We provide the total computation time for each experiment and type of resources we used.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See Section 4.1}.
  \item Did you mention the license of the assets?
    \answerYes{See Appendix.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We include the URL for our code.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
%   Even if you used an existing dataset, you should check how data was collected and whether consent was obtained. We acknowledge this might be difficult, so please try your best; the goal is to raise awareness of possible issues that might be ingrained in our community.
    \answerYes{See Appendix.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{See Appendix.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{We neither use crowdsourcing nor conduct research with human subjects.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{We neither use crowdsourcing nor conduct research with human subjects.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{We neither use crowdsourcing nor conduct research with human subjects.}
\end{enumerate}

\end{enumerate}



==> tables/__data_stats.tex <==

\begin{table}
\centering
\small
% \begin{tabular}{l|rrr}
\renewcommand{\arraystretch}{1.1}
\caption{\textbf{Basic statistics of benchmark datasets.} \sr{how about describing these in text?}
\sr{I think that table is OK but there are too many tables in this paper.}
\jb{It is my first consideration but I think the table-way is better for brevity but I think so too describing in text is more natural.} 
\sr{Actually, I wonder where the domain gaps comes from. For example, extracting different source datasets or gathering different environments.. } \jb{Good point. I will try to write this table into text with description about that.}}
\begin{tabular}{l|rrr}
\toprule
Dataset   & {\#Domains} & {\#Classes} & {\#Data}  \\
\midrule
\data{PACS}           & 4                              & 7                              & $9,991$                                \\
\data{VLCS}           & 4                              & 5                              & $10,729$                               \\
\data{OfficeHome}     & 4                              & 65                             & $15,588$                               \\
\data{TerraIncognita} & 4                              & 10                             & $24,788$                               \\
\data{DomainNet}      & 6                              & 345                            & $586,575$                             \\
\bottomrule
\end{tabular}
\label{table:data_stats}
\end{table}
